dPMP-Deep Probabilistic Motion Planning: A use case in Strawberry Picking Robot

This paper presents a novel probabilistic approach to deep robot learning from demonstrations (LfD). Deep movement primitives (DMPs) are deterministic LfD model that maps visual information directly into a robot trajectory. This paper extends DMPs and presents a deep probabilistic model that maps the visual information into a distribution of effective robot trajectories. The architecture that leads to the highest level of trajectory accuracy is presented and compared with the existing methods. Moreover, this paper introduces a novel training method for learning domain-specific latent features. We show the superiority of the proposed probabilistic approach and novel latent space learning in the lab's real-robot task of strawberry harvesting. The experimental results demonstrate that latent space learning can significantly improve model prediction performances. The proposed approach allows to sample trajectories from distribution and optimises the robot trajectory to meet a secondary objective, e.g. collision avoidance.

==> images.tex <==

\begin{flushleft}
\begin{table}[!t]
\vspace{.3cm}
\centering
\caption{Joint space predictions.\\ deep-ProMp-cVAE is the most accurate model.}
\label{table:joint}
\begin{tabular}{@{}cccccc@{}}
\multirow{2}{*}{Joint} & deep-ProMP-AE & \multicolumn{2}{c}{deep-ProMP-VAE} & \multicolumn{2}{c}{deep-ProMP-cVAE}\\
& RMSE & RMSE & drop  & RMSE & drop\\
\toprule
J1 &  5.4$\times 10^{-4}$  & 1.3$\times 10^{-4}$ & -74\% & 1.0$\times 10^{-4}$ & -28\%\\
J2 &  48.9$\times 10^{-4}$ & 14.4$\times 10^{-4}$ & -70\% & 9.0$\times 10^{-4}$ & -38\% \\
J3 &  93.0$\times 10^{-4}$ & 9.6$\times 10^{-4}$ & -89\% & 5.9$\times 10^{-4}$ & -38\% \\
J4 &  37.1$\times 10^{-4}$ & 19.3$\times 10^{-4}$ & -47\% & 5.9$\times 10^{-4}$ & -71\% \\
J5 &  24.2$\times 10^{-4}$ & 23.5$\times 10^{-4}$ & -2.7\% & 20.1$\times 10^{-4}$ & -13\% \\
J6 &  29.0$\times 10^{-4}$ & 15.4$\times 10^{-4}$& -48\% & 15.4$\times 10^{-4}$ & -0\% \\
J7 &  21.4$\times 10^{-4}$ & 5.4$\times 10^{-4}$ & -75\% & 5.4$\times 10^{-4}$ & -0\% \\
\bottomrule
\end{tabular}
\end{table}
\end{flushleft}
%%%% <<<<<<<<<<. >>>>>>>>>>


\begin{figure*}[t!]
  \includegraphics[width=.85\linewidth]{images/latent.png}
  \centering
  \caption{Latent space visualisation/representation through T-SNE embedding before and after domain specific tuning.  After tuning, the clustering in the embedding space increases in both AE and VAE. A numerical evaluation is present in Table \ref{table:latent}.}
\label{fig:latent_Space}
\end{figure*}

\begin{flushleft}
\begin{table}[tb!]
\centering
\caption{Cluster separability of latent space representation through T-SNE using Davies-Bouldin Index before and after latent space tuning with . A lower score indicates better clustering. Fig. \ref{fig:latent_Space} shows the T-SNE visualisations}
\label{table:latent}
\begin{tabular}{cc|c}
\multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{\textbf{Davies-Bouldin score}} \\
\multicolumn{1}{c|}{\multirow{2}{*}{AE}}  & base               & 0.616 \\
\multicolumn{1}{c|}{}                     & \textbf{latent space tuned} & $\mathbf{0.482}$ \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{VAE}} & base               & 0.424 \\
\multicolumn{1}{c|}{}                     & \textbf{latent space tuned} & $\mathbf{0.352}$
\end{tabular}
\end{table}
\end{flushleft}


   


\begin{table*}[!tbh]
\centering
\vspace{.3cm}
\caption{Joint space vs Task Space prediction accuracy at the final point. Task space predictions are more accurate.}
\label{table:joint_vs_task}
\begin{tabular}{ccccc|cccc}
 &
  \multicolumn{4}{c|}{joint space prediction} &
  \multicolumn{4}{c}{task space prediction} \\ \cline{2-9} 
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{mean} &
  \multicolumn{2}{c|}{3std.} &
  \multicolumn{2}{c|}{mean} &
  \multicolumn{2}{c|}{3std.} \\
\multicolumn{1}{c|}{} &
  position [-] &
  \multicolumn{1}{c|}{orientation [-]} &
  position [-] &
  orientation [-] &
  position [-] &
  \multicolumn{1}{c|}{orientation [-]} &
  position [-] &
  \multicolumn{1}{c|}{orientation [-]} \\ \hline
\multicolumn{1}{c|}{deep-ProMP-Direct} &
  0.15 &
  \multicolumn{1}{c|}{0.1} &
  0.31 &
  0.41 &
  0.08 &
  \multicolumn{1}{c|}{0.06} &
  0.10 &
  \multicolumn{1}{c|}{0.10} \\
\multicolumn{1}{c|}{deep-ProMP-AE} &
  0.10 &
  \multicolumn{1}{c|}{0.06} &
  0.32 &
  0.41 &
  0.04 &
  \multicolumn{1}{c|}{0.04} &
  0.09 &
  \multicolumn{1}{c|}{0.07} \\
\multicolumn{1}{c|}{deep-ProMP-VAE} &
  0.06 &
  \multicolumn{1}{c|}{0.03} &
  0.19 &
  0.31 &
  0.03 &
  \multicolumn{1}{c|}{0.03} &
  0.07 &
  \multicolumn{1}{c|}{0.06} \\
\multicolumn{1}{c|}{deep-ProMP-cVAE} &
  0.04 &
  \multicolumn{1}{c|}{0.02} &
  0.18 &
  0.28 &
  0.02 &
  \multicolumn{1}{c|}{0.02} &
  0.06 &
  \multicolumn{1}{c|}{0.06}
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%<<<<<<<<<<<>>>>>>>>>
\begin{flushleft}
\begin{figure}[tb]
\begin{center}
  \includegraphics[width=1\linewidth]{performances_real_robot_graph.png}
\end{center}
  \caption{Experimental results from the implementation on the real robot. It is visible that performances increase going from Deep-ProMP-AE to deep-ProMP-VAE to Deep-ProMP-cVAE. A further improvement can be noticed after the domain-specific training of the encoders. Finally it is evident that the mean trajectory leads to higher precision in the final point with respect to the other sampled trajectories. }
\label{fig:results}
\end{figure}
\end{flushleft}
%%%%%%%%%%%%%%%<<<<<<<<<<<>>>>>>>>>

